Which Shortcut Cues Will DNNs Choose? A Study from the Parameter-Space Perspective

Deep neural networks (DNNs) often rely on easy-to-learn discriminatory features, or cues, that are not necessarily essential to the problem at hand. For example, ducks in an image may be recognized based on their typical background scenery, such as lakes or streams. This phenomenon, also known as shortcut learning, is emerging as a key limitation of the current generation of machine learning models. In this work, we introduce a set of experiments to deepen our understanding of shortcut learning and its implications. We design a training setup with several shortcut cues, named WCST-ML, where each cue is equally conducive to the visual recognition problem at hand. Even under equal opportunities, we observe that (1) certain cues are preferred to others, (2) solutions biased to the easy-to-learn cues tend to converge to relatively flat minima on the loss surface, and (3) the solutions focusing on those preferred cues are far more abundant in the parameter space. We explain the abundance of certain cues via their Kolmogorov (descriptional) complexity: solutions corresponding to Kolmogorov-simple cues are abundant in the parameter space and are thus preferred by DNNs. Our studies are based on the synthetic dataset DSprites and the face dataset UTKFace. In our WCST-ML, we observe that the inborn bias of models leans toward simple cues, such as color and ethnicity. Our findings emphasize the importance of active human intervention to remove the inborn model biases that may cause negative societal impacts.

==> chapters/tmp.tex <==

\begin{figure}[h]
    \centering
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/fft_training_comparison_shape_scale_orientation_color.pdf}
		\vspace{-1em}
		\caption{FFnet}
		\label{fig:res_colordsprites:FFnet}
	\end{subfigure} 
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/resnet_training_comparison_shape_scale_orientation_color.pdf}
		\vspace{-1em}
		\caption{ResNet20}
		\label{fig:res_colordsprites:conv}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/vit_training_comparison_shape_scale_orientation_color.pdf}
		\vspace{-1em}
		\caption{VIT}
		\label{fig:res_colordsprites:resnet}
	\end{subfigure} 
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/fft_training_comparison_shape_scale_orientation.pdf}
		\vspace{-1em}
		\caption{FFnet}
		\label{fig:res_colordsprites:FFnet}
	\end{subfigure} 
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/resnet_training_comparison_shape_scale_orientation.pdf}
		\vspace{-1em}
		\caption{ResNet20}
		\label{fig:res_colordsprites:conv}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/vit_training_comparison_shape_scale_orientation.pdf}
		\vspace{-1em}
		\caption{VIT}
		\label{fig:res_colordsprites:resnet}
	\end{subfigure} 
	\caption{Figures (a)-(b)-(c) show the results of training respectively a FFnet, ResNet20 and VIT architectures on the DLS composed of the $\{shape, scale, orientation, color\}$ set in ColorDSprites, and testing them on the respective off-diagonal test sets of the corresponding features. Figures (d)-(e)-(f) show the results of training respectively a FFnet, ResNet20 and VIT architectures on the DLS composed of the $\{shape, scale, orientation\}$ set in ColorDSprites, and testing them on the respective off-diagonal test sets of the corresponding features.}
	\label{fig:res_colordsprites}
\end{figure}



\begin{figure}[h]
    \centering
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/fft_training_comparison_age_gender_ethnicity.pdf}
		\vspace{-1em}
		\caption{FFnet}
		\label{fig:res_colordsprites:FFnet}
	\end{subfigure} 
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/resnet_training_comparison_age_gender_ethnicity.pdf}
		\vspace{-1em}
		\caption{ResNet20}
		\label{fig:res_colordsprites:conv}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/vit_training_comparison_age_gender_ethnicity.pdf}
		\vspace{-1em}
		\caption{VIT}
		\label{fig:res_colordsprites:resnet}
	\end{subfigure} 
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/fft_training_comparison_age_gender.pdf}
		\vspace{-1em}
		\caption{FFnet}
		\label{fig:res_colordsprites:FFnet}
	\end{subfigure} 
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/resnet_training_comparison_age_gender.pdf}
		\vspace{-1em}
		\caption{ResNet20}
		\label{fig:res_colordsprites:conv}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\includegraphics[width=\linewidth]{figures/vit_training_comparison_age_gender.pdf}
		\vspace{-1em}
		\caption{VIT}
		\label{fig:res_colordsprites:resnet}
	\end{subfigure} 
	\caption{Figures (a)-(b)-(c) show the results of training respectively a FFnet, ResNet20 and VIT architectures on the DLS composed of the $\{ethnicity, gender, age\}$ set in ColorDSprites, and testing them on the respective off-diagonal test sets of the corresponding features. figures (d)-(e)-(f) show the results of training respectively a FFnet, ResNet20 and VIT architectures on the DLS composed of the $\{gender, age\}$ set in ColorDSprites, and testing them on the respective off-diagonal test sets of the corresponding features.}
	\label{fig:res_UTKface}
\end{figure}



% Vanilla learning algorithms trained on data with multiple feasible cues are inevitably biased to simple cues. There must be an active fix on the training data \citep{li2018resound,li2019repair,stylizedimagenet,mimetics}, learning algorithm \citep{clark2019learnedmixin,bahng2019rebias,adversarially_fair_representation}, and post-inference calibration \citep{fairness_calibration,black_box_postprocessing_fairness} to make the generalisable and ethical cues more attractive to models.



\section{Related work}
\label{sec:related}

What shapes feature representations?
Exploring datasets, architectures, and training

DiagViB-6: A Diagnostic Benchmark Suite for Vision Models in the Presence of Shortcut and Generalization Opportunities

Shortcut Learning in Deep Neural Networks

\paragraph{Setups for analysing shortcut bias.}



\paragraph{Why shortcut bias.}

...
